Guided Safe Shooting: model based reinforcement learning with safety constraints

In the last decade, reinforcement learning successfully solved complex control tasks and decision-making problems, like the Go board game. Yet, there are few success stories when it comes to deploying those algorithms to real-world scenarios. One of the reasons is the lack of guarantees when dealing with and avoiding unsafe states, a fundamental requirement in critical control engineering systems. In this paper, we introduce Guided Safe Shooting (GuSS), a model-based RL approach that can learn to control systems with minimal violations of the safety constraints. The model is learned on the data collected during the operation of the system in an iterated batch fashion, and is then used to plan for the best action to perform at each time step. We propose three different safe planners, one based on a simple random shooting strategy and two based on MAP-Elites, a more advanced divergent-search algorithm. Experiments show that these planners help the learning agent avoid unsafe situations while maximally exploring the state space, a necessary aspect when learning an accurate model of the system. Furthermore, compared to model-free approaches, learning a model allows GuSS reducing the number of interactions with the real-system while still reaching high rewards, a fundamental requirement when handling engineering systems.

==> Algos.tex <==
% ==================================  MBRL
% \begin{figure}[!h]
% %\renewcommand{\algotab}[0]{\hspace*{\labelsep}}
% \setlength{\algoitemsep}{0pt}
% %\setlength{\algowidth}{1\columnwidth}
% \centerline{
% \begin{myalgorithm}{$\Algo{IteratedMBRL}(p_\text{real}, \cS_0,  N, T)$:}
% \Aitem \Algo{Choices}: $\pi^{(0)}$, $\hat{p}^{(0)}$, \Algo{Model}, \Algo{Actor}
% \Aitem $\bs_1 \rLeadsto \cS_0$ \mt \algoremark{draw initial state}
% \Aitem $\cT^{(1)} \setto \Algo{Rollout}\left(\pi^{(0)}, p_\text{real}, \bs_1, T\right)$ \mt \algoremark{random trace}
% \Aitem \For $\tau \setto 1$ \To $N$: \algoremark{for $N$ episodes}
% \Aitem \mt $\hat{p}^{(\tau)} \setto \Algo{Model}\big(\bigcup_{\tau^\prime=1}^\tau \cT^{(\tau^\prime)}, \hat{p}^{(\tau - 1)}\big)$\\ \mt \algoremark{learn system model} \label{linModelUpdate}
% \Aitem \mt $\pi^{(\tau)} \setto  \Algo{Actor}\left(\pi^{(0)}, \pi^{(\tau-1)}, \hat{p}^{(\tau)}, \bigcup_{\tau^\prime=1}^\tau \cT^{(\tau)}\right)$ \\ \mt \algoremark{initiating \Algo{Actor} by calling \Algo{Actor.Init()}} \label{linPolicyUpdate}
% \Aitem \mt $\bs_1 \rLeadsto \cS_0$  \algoremark{draw initial state}
% \Aitem \mt $\cT^{(\tau+1)} \setto  \Algo{Rollout}\left(\pi^{(\tau)}, p_\text{real}, \bs_1, T\right)$ \algoremark{new trace} \label{linEpisodeTrace}
% \Aitem \Return $\pi^{(N)}$, $\hat{p}^{(N)}$, $\bigcup_{\tau=1}^N \cT^{(\tau)}$
% \end{myalgorithm}
% }
% \caption[]{\textbf{The iterated batch MBRL loop.}
% Starting from an initial (typically random) policy $\pi^{(0)}$ and system model $\hat{p}^{(0)}$, we alternate between learning the model (Line~\ref{linModelUpdate}) and initializing the policy as an instance of \Algo{Actor} (Line~\ref{linPolicyUpdate}). 
% In each episode $\tau$, we roll out a new trace $\cT^{(\tau+1)}$ and add it to the buffer of transitions. Model learning is described in Section~\ref{sec:method}, and the QD actor is defined in Section~\ref{sec:me} and in Fig~\ref{figQDActor}. 
% The subroutine \Algo{Rollout} is defined in Appendix \ref{app:pseudocode}, Fig~\ref{figRollout}.\\
% \textbf{Input parameters:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $p_\text{real}: (\bs_t, \ba_t) \Leadsto \bs_{t+1}$: the real system (transition dynamics). It is assumed to be slow so Line~\ref{linEpisodeTrace} is what dominates the execution time.
%     \item $\cS_0$: distribution of the real system's initial state. 
%     \item $N$: number of episodes.
%     \item $T$: length of episodes.
% \end{itemize}
% \textbf{Algorithmic choices:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $\pi^{(0)}: \bs_t \Leadsto \ba_t$: an initial (typically random) policy. \item $\hat{p}^{(0)}: (\bs_t, \ba_t) \Leadsto \bs_{t+1}$, an initial system model (typically a randomly initialized network).
%     \item \Algo{Model}: a supervised learning (probabilistic or deterministic time-series forecasting) model. It can either be trained from scratch on the collected traces $\bigcup_{\tau^\prime=1}^\tau \cT^{(\tau)}$, or continually updated from the  previous system model $\hat{p}^{(\tau-1)}$.
%     \item \Algo{Actor}: a policy learning algorithm (Fig~\ref{figQDActor}) that typically updates $\pi^{(\tau-1)}$ using the model $\hat{p}^{(\tau)}$. It can also use the initial (usually random) policy $\pi^{(0)}$, typically in the background-planning loop (e.g., the random shooting \Algo{RSActor} in Appendix \ref{app:pseudocode}, Fig~\ref{figActors}). 
% \end{itemize}
% \label{figMBRL}}
% \end{figure}

% ==================================================
% QD ACTOR

% \begin{figure}[!h]
% \setlength{\algoitemsep}{0pt}
% \centerline{
% \begin{myalgorithm}{$\Algo{QualityDiversityActor}\big(\pi^{(0)}, \pi^\text{prev}, p\big)$:}
% \Aitem \Algo{Choices}: \Algo{QDInit}, \Algo{QDMutate}, \Algo{QDSelect}, \Algo{TrajOpt}, $L$, $n$, $n_\text{new}$, $m$, $M$
% \Aitem \Algo{Init()}:
% \Aitem \mt $\frR \setto  \Algo{QDInit}\big(\pi^{(0)}, \pi^\text{prev}, n\big)$ \mt \algoremark{initial pool} \label{linQDInit}
% \Aitem $\Algo{Act}(\bs)$:
% \Aitem \mt $\frT \setto \Algo{MultiRollout}\big(\frR, p, \bs, L, m\big)$
% \Aitem \mt \For $j \setto 1$ \To $M$: \mt \algoremark{$M$ generations}
% \Aitem \mtt $\frR_\text{new} \setto \Algo{QDMutate}(\frR, n_\text{new})$ \mt \algoremark{mutate policies} \label{linQDMutate}
% \Aitem \mtt $\frT_\text{new} \setto \Algo{MultiRollout}\big(\frR_\text{new}, p, \bs, L, m\big)$
% \Aitem \mtt $\frR \setto \frR \cup \frR_\text{new}$
% \Aitem \mtt $\frT \setto \frT \cup \frT_\text{new}$
% \Aitem \mtt $\frR, \frT \setto \Algo{QDSelect}\big(\frR, \frT\big)$ \mt \algoremark{delete policies} \label{linQDSelect}
% \Aitem \mt \Return $\Algo{TrajOpt}(\frT)$ \algoremark{planning} \label{lineTOpt}
% \end{myalgorithm}
% }
% \caption[]{\textbf{The quality diversity actor.}
% The QD actor initializes a pool of policies, evolves them using mutation and selection operators for $M$ generations, evaluating them through rollouts on the transition dynamics model, and uses them for planning.\\
% \textbf{Input parameters:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $\pi^{(0)}: \bs_t \Leadsto \ba_t$: initial (typically random) policy.
%     \item $\pi^\text{prev}: \bs_t \Leadsto \ba_t$: the policy from the previous epoch, in case the actor wants to build on it.
%     \item $p: (\bs_t, \ba_t) \Leadsto \bs_{t+1}$: a transition dynamics, typically a learned system model.
% \end{itemize}
% \textbf{Algorithmic choices:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item \Algo{QDInit}: the algorithm to create $n$ initial QD planning policies (planners). Alternatively, it can keep the pool from the previous epoch.
%     \item \Algo{QDMutate}: the algorithm to create new mutated planners by perturbing $n_\text{new}$ planners randomly selected from the pool $\frR$.
%     \item \Algo{QDSelect}: the algorithm to select safe planners by deleting grid collisions (Fig.~\ref{figSafeMESelector}).
%     \item \Algo{TrajOpt}: the algorithm to select the best trajectory from $\frT$ and return its first action (Fig.~\ref{figSafeTrajOpt}).
%     \item $L$: the length of planning trajectories (\emph{horizon}).
%     \item $n$: the size of the initial pool.
%     \item $n_\text{new}$: the number of new mutations generated at each generation.
%     \item $m$: the number of particles.
%     \item $M$: the number of evolutionary generations.
% \end{itemize}
% \label{figQDActor}}
% \end{figure}

% =================================================

% SAFE SELECT
% \begin{figure}[!h]
% %\renewcommand{\algotab}[0]{\hspace*{\labelsep}}
% \setlength{\algoitemsep}{0pt}
% \centerline{
% \begin{myalgorithm}{$\Algo{SafeMAPElitesSelect}\\ \mt \big(\frR = [\rho_i]_{i=1}^n, \frT = [\cT_{i,j}]_{i=1..n}^{j=1..m}\big)$:}
% \Aitem \Algo{Choices}: , \Algo{Value}, \Algo{Cost}, $f$
% \Aitem $[V_i]_{i=1}^n \setto [\Algo{Value}(\cT_{i,\cdot})]_{i=1}^n$ \algoremark{values}
% \Aitem $[C_i]_{i=1}^n \setto [\Algo{Cost}(\cT_{i,\cdot})]_{i=1}^n$ \algoremark{costs}
% \Aitem $[\bar{b}_i]_{i=1}^n \setto [f(\cT_{i,\cdot})]_{i=1}^n$ \algoremark{grid behavior descriptors}
% \Aitem \For $i \setto 1$ \To $n$: \mt \algoremark{filter collisions}
% \Aitem \mt \If $\exists i' \not= i: \bar{b}_{i'} = \bar{b}_i \wedge C_{i'} < C_i$:
% \Aitem \mtt $\frR \setto \frR - \{\rho_i\}$ \mt \algoremark{delete planner}
% \Aitem \mt \If $\exists i' \not= i: \bar{b}_{i'} = \bar{b}_i \wedge \big(V_{i'} > V_i \vee (V_{i'} = V_i \wedge i' < i)\big)$:
% \Aitem \mtt $\frR \setto \frR - \{\rho_i\}$ \mt \algoremark{delete planner}
% \Aitem \Return $\frR$ \algoremark{updated pool of planners}
% \end{myalgorithm}
% }
% \caption[]{\textbf{The safe MAP-Elites selector} maps the rollout traces $[\cT_{i,\cdot}]_{i=1}^{n}$ onto a finite grid $\bar{\cB}$. If there is a collision, it first keeps the policies with the lowest safety cost, then it deletes the suboptimal policies in each grid cell (it keeps at most one policy per cell with the highest value; if there is a tie it keeps the policy with the lowest index).\\
% \textbf{Input parameters:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $[\rho_i]_{i=1}^n$: current QD pool of planners.
%     \item $[\cT_i]_{i=1}^n$: rollouts of the current pool of planners on the model.
% \end{itemize}
% \textbf{Algorithmic choices:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $\Algo{Value}$: function that measures the value of a trajectory (Appendix \ref{app:pseudocode}, Fig~\ref{figValues}).
%     \item $\Algo{Cost}$: function that measures the safety cost of a trajectory.
%     \item $f$: behavior mapping from rollout traces to the feature space $\bar{\cB}$. It does both the feature mapping and discretization to a finite grid to generate collisions of similar policies in the pool.
% \end{itemize}
% \label{figSafeMESelector}}
% \vspace{-0.5cm}
% \end{figure}


% ====================================

% \section{Pseudo-codes of additional routines} 
%  \label{app:pseudocode}
% \subsection{Map-Elites selector}
% \begin{figure}[!ht]
% %\renewcommand{\algotab}[0]{\hspace*{\labelsep}}
% \setlength{\algoitemsep}{0pt}
% \centerline{
% \begin{myalgorithm}{$\Algo{MAPElitesSelect}\big(\frR = [\rho_i]_{i=1}^n, \frT = [\cT_{i,j}]_{i=1..n}^{j=1..m}\big)$:}
% \Aitem \Algo{Choices}: \Algo{Value}, $f$
% \Aitem $[V_i]_{i=1}^n \setto [\Algo{Value}(\cT_{i,\cdot})]_{i=1}^n$ \algoremark{values}
% \Aitem $[\bar{b}_i]_{i=1}^n \setto [f(\cT_{i,\cdot})]_{i=1}^n$ \algoremark{grid behavior descriptors}
% \Aitem \For $i \setto 1$ \To $n$: \mt \algoremark{filter collisions}
% \Aitem \mt \If $\exists i' \not= i: \bar{b}_{i'} = \bar{b}_i \wedge \big(V_{i'} > V_i \vee (V_{i'} = V_i \wedge i' < i)\big)$:
% \Aitem \mtt $\frR \setto \frR - \{\rho_i\}$ \mt \algoremark{delete planner}
% \Aitem \Return $\frR$ \algoremark{updated pool of planners}
% \end{myalgorithm}
% }
% \caption[]{\textbf{The MAP-Elites selector}  maps the rollout traces $[\cT_{i,\cdot}]_{i=1}^{n}$ onto a finite grid $\bar{\cB}$ and deletes the suboptimal policies in each grid cell (it keeps at most one policy per cell with the highest value; if there is a tie it keeps the policy with the lowest index).\\
% \textbf{Input parameters:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $\frR = [\rho_i]_{i=1}^n$: the current QD pool of planners.
%     \item $\frT = [\cT_{i,j}]_{i=1..n}^{j=1..m}$: the rollouts of the current pool of planners on the model.
% \end{itemize}
% \textbf{Algorithmic choices:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $\Algo{Value}$: The function that measures the value of a trajectory (Fig~\ref{figValues}).
%     \item $f$: the behavior mapping from rollout traces to the feature space $\bar{\cB}$. It does both the feature mapping and discretization to a finite grid to generate collisions of similar policies in the pool.
% \end{itemize}
% \label{figMESelector}}
% \vspace{-0.5cm}
% \end{figure}

% \subsection{Random shooting Actor}

% \begin{figure}[!h]
% %\renewcommand{\algotab}[0]{\hspace*{\labelsep}}
% \setlength{\algoitemsep}{0pt}
% \centerline{
% \begin{myalgorithm}{$\Algo{RSActor}\big(\pi^{(0)}, \pi^\text{prev}, p\big)$:}
% \Aitem \Algo{Choices}: $L$, $n$, $m$
% \Aitem \Algo{Init()}:
% \Aitem \mt \Algo{Pass}
% \Aitem $\Algo{Act}(\bs)$:
% \Aitem \mt $\frT \setto \Algo{MultiRollout}\big([\pi^{(0)}]_{i=1}^n, p, \bs, L, m\big)$ \algoremark{traces}
% \Aitem \mt \Return $\Algo{TrajOpt}(\frT)$ \algoremark{planning}
% \end{myalgorithm}
% }
% \caption[]{\textbf{Random shooting actor (policy executed on the real system).}
% \Algo{RSActor} is a classical random shooting planner that uses the random policy $\pi^{(0)}$ for all rollouts (Fig~\ref{figRollout}) and planning (Fig~\ref{figTrajOpt}).}
% \label{figActors}
% \end{figure}


% \textbf{Input parameters:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $\pi^{(0)}: \bs_t \Leadsto \ba_t$: initial (typically random) policy.
%     \item $\pi^\text{prev}: \bs_t \Leadsto \ba_t$: the policy from the previous epoch, in case the actor wants to build on it.
%     \item $p: (\bs_t, \ba_t) \Leadsto \bs_{t+1}$: a transition dynamics, typically a learned system model.
% \end{itemize}
% \textbf{Algorithmic choices:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $L$: the length of planning trajectories (\emph{horizon}).
%     \item $n$: the number of planning trajectories.
%     \item $m$: the number of particles.
% \end{itemize}




% \subsection{Trajectory optimization}
% \begin{figure}[!ht]
% %\renewcommand{\algotab}[0]{\hspace*{\labelsep}}
% \setlength{\algoitemsep}{0pt}
% \centerline{
% \begin{myalgorithm}{$\Algo{TrajOpt}\big(\frT = [\cT_{i,j}]_{i=1..n}^{j=1..m}\big)$:}
% \Aitem \Algo{Choices}: \Algo{Value}
% \Aitem \For $i \setto 1$ \To $n$:
% \Aitem \mt $V_i \setto \Algo{Value}\big(\cT_{i,\cdot}\big)$ \mt \algoremark{total reward of $\cT_i$} \label{linValue} 
% \Aitem $i^* \setto \argmax_i V_i$ \mtt \algoremark{index of the best trace} \label{linBestTrace}
% \Aitem \Return $\ba_1^{(i^*)}$   \algoremark{first action of the best trace $\cT_{i^*}$}
% \end{myalgorithm}
% }
% \caption[]{\textbf{Shooting trajectory optimization.} \Algo{TrajOpt} is a classical planner that returns the first action of the best trajectory in the rollouts $[\cT_i]_{i=1}^n$.}

% \textbf{Input parameters:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $\frT = [\cT_{i,j}]_{i=1..n}^{j=1..m}$: a set of rollout trajectories with $n$ rollouts and $m$ particles in each.
% \end{itemize}
% \textbf{Algorithmic choices:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $\Algo{Value}$: The function that measures the value of a trajectory (Fig~\ref{figValues}).
%     \item $\Algo{Cost}$: The function that measures the safety cost of a trajectory.
% \end{itemize}
% \label{figTrajOpt}
% \end{figure}

% \newpage
% \begin{figure}[!ht]
% %\renewcommand{\algotab}[0]{\hspace*{\labelsep}}
% \setlength{\algoitemsep}{0pt}
% \centerline{
% \begin{myalgorithm}{$\Algo{SafeTrajOpt}\big(\frT = [\cT_{i,j}]_{i=1..n}^{j=1..m}\big)$:}
% \Aitem \Algo{Choices}: \Algo{Value}, \Algo{Cost}
% \Aitem \For $i \setto 1$ \To $n$:
% \Aitem \mt $V_i \setto \Algo{Value}\big(\cT_{i,\cdot}\big)$ \mt \algoremark{total reward of $\cT_{i,\cdot}$}
% \Aitem \mt $C_i \setto \Algo{Cost}\big(\cT_{i,\cdot}\big)$ \mt \algoremark{total cost of $\cT_i$}
% \Aitem $\cI^* \setto \argmin_{i=1}^n C_i$ \mt \algoremark{indices of lowest cost traces} \Aitem $i^* \setto \argmax_{i \in \cI^*} V_i$ \mt \algoremark{index of the best safe trace} %\label{linBestTrace}
% \Aitem \Return $\ba_1^{(i^*)}$ \algoremark{first action of the best trace $\cT_{i^*}$}
% \end{myalgorithm}
% }
% \caption[]{\textbf{Safe trajectory optimization.} \Algo{SafeTrajOpt} returns the first action of the best trajectory from among those with the lowest cost in the rollouts $[\cT_i]_{i=1}^n$.}

% \textbf{Input parameters:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $\frT = [\cT_{i,j}]_{i=1..n}^{j=1..m}$: a set of rollout trajectories with $n$ rollouts and $m$ particles in each.
% \end{itemize}
% \textbf{Algorithmic choices:}
% \begin{itemize}
%     \setlength{\itemsep}{0pt}
%     \item $\Algo{Value}$: The function that measures the value of a trajectory (Appendix \ref{app:pseudocode}, Fig~\ref{figValues}).
%     \item $\Algo{Cost}$: The function that measures the safety cost of a trajectory.
% \end{itemize}
% \label{figSafeTrajOpt}
% \end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/background.tex <==
\section{Background}
\label{sec:background}
In this section, we introduce the concepts of safe-\gls{rl} and \gls{qd} algorithms on which our method builds.

\subsection{Safe Reinforcement Learning}
Reinforcement learning problems are usually represented as a Markov decision process (MDP) $\mathcal{M} = \langle  \mathcal{S},   \mathcal{A},   \mathcal{T}, r, \gamma \rangle$, where   $\mathcal{S}$ is the state space, $\mathcal{A}$ is the action space, $\mathcal{T} : \mathcal{S} \times \mathcal{A} \rightarrow \mathcal{S}$ is the transition dynamics,  $r : \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ is the reward function and $\gamma \in [0,1]$ is the discount factor. Let $\Delta(\mathcal{X})$ denote the family of distributions over a set $\mathcal{X}$. The goal is to find a policy $\pi : \mathcal{S} \rightarrow \Delta(\mathcal{A}) $
which maximizes the expected discounted return $\pi^* = \underset{\pi}{\arg\max}$ $\mathbb{E}_\pi \left[  \sum_{t}^{} \gamma^t r(s_t,a_t) \right]$ \citep{sutton2018reinforcement}. 
This formulation can be easily accommodated to incorporate constraints, for example representing safety requirements. 
To do so, similarly to the reward function, we define a new cost function $\mathcal{C} : \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$  which, in our case, is a simple indicator for whether an unsafe interaction has occurred ($\mathcal{C}_t=1$ if the state is unsafe and $\mathcal{C}_t=0$ otherwise).
The new goal is then to find an optimal policy $\pi^*$ with a high expected reward $\mathbb{E}_\pi\left[  \sum_{t}^{} \gamma^tr(s_t,a_t) \right]$ and a low safety cost $\mathbb{E}_\pi \left[\sum_{t}^{} C(s_t,a_t) \right]$.
%\begin{equation}
%    \begin{cases}
%        {\max}~\mathbb{E}_\pi\left[  %\sum_{t}^{} \gamma^tr(s_t,a_t) \right] \\
%        {\min}~\mathbb{E}_\pi \left[  %\sum_{t}^{} C(s_t,a_t) \right]\\
%    \end{cases}
%\end{equation}
One way to solve this new problem  is to rely on constrained Markov Decision processes (CMDPs) \citep{altman1999constrained} by adding constraints on the expectation \citep{la2013actor} or on the variance of the return \citep{chow2017risk}. 

\subsection{Model Based Reinforcement Learning}
In this work, we address the issue of respecting safety constraints through an \gls{mbrl} approach \citep{moerland2021survey}. 
In this setting, the transition dynamics $p_{\text{real}}$ are estimated using the data collected when interacting with the real system.
The objective is to learn a model $p(s_t, a_t) \rightsquigarrow s_{t+1}$\footnote{We use $\rightsquigarrow$ to denote both probabilistic and deterministic mapping.} to predict $s_{t+1}$ given $s_t$ and $a_t$ and use it  to learn an optimal policy  $\pi^*$. 
In this work, we considered the iterated-batch learning approach (also known as growing batch \citep{lange2012batch} or semi-batch \citep{singh1994reinforcement}).
In this setting, the model is trained and evaluated on the real-system through an alternating two-step process consisting in:
(i) applying and evaluating the learned policy on the environment for a whole episode and 
(ii) then training the model on the growing data  of transitions collected during the evaluation $\tau$ itself $\mathcal{T}r_t = \{(s_1,a_1, r_1,c_1,s'_1)^0, \dots, (s_t,a_t, r_t,c_t,s'_t)^0, \dots, (s_1,a_1, r_1,c_1,s'_1)^\tau, \dots, (s_t,a_t, r_t,c_t,s'_t)^{\tau}\}$ and updating the policy.
The process is repeated until a given number of evaluations or a certain model precision is reached.

\subsection{Quality Diversity}
\label{sec:me}

\gls{qd} methods are a family of \gls{ea} performing divergent search with the goal of generating a collection of diverse but highly performing policies \citep{pugh2016quality, cully2017quality}.
The divergent search is performed over a, usually hand-designed, \emph{behavior space} $\mathcal{B}$ in which the behavior of the evaluated policies is represented.
Some of these methods have been shown, given enough iterations, to be able to uniformly cover the whole behavior space \citep{doncieux2019novelty}.
Combining these methods with \gls{rl} approaches then allows to greatly increase the exploration abilities of \gls{rl} algorithms.

Among the different \gls{qd} methods introduced in the literature  \citep{lehman2011evolving, paolo2021sparse, mouret2015illuminating}, in this work we use the \gls{me} algorithm \citep{mouret2015illuminating} due to its simplicity and power.
A detailed description of how \gls{me} works and the related pseudo-code are presented in Appendix \ref{app:me}.

==> sections/conclusion.tex <==
\section{Conclusion and Future work}
\label{sec:conclusion}
In this study, we proposed \gls{name}, a model based planning method for safe reinforcement learning. 
We tested the method on three environments with safety constraints and the results show that, while being simple, \gls{name} provides good results in terms of both safety and reward trade-off with minimal computational complexity. 
Moreover, we observed that in some settings, like Safe Pendulum, the introduction of safety constraints can lead to a better completion of the task.
Further experiments are needed to confirm this effect, but if this holds, it could be possible to take advantage of it in a curriculum learning fashion: starting from strict safety constraints and incrementally relaxing them to get to the final task and safety requirement. 
This could help even more in the application of \gls{rl} methods to real engineering systems, allowing the engineers handling the system to be more confident in the performances of the methods.

Notwithstanding the great results obtained by our proposed approach, the performances of \gls{name} are still tied to the accuracy of the model.
If the model is wrong, it could easily lead the agent to unsafe states.
This is particularly noticeable in the Safe Car Goal environment, with the high cost notwithstanding the high reward.
As discussed in Section \label{sec:discussion}, these results require more in depth analysis, but also open the path to new directions of research.
A possible solution to the problem of the model inaccuracy is to have uncertainty aware models that can predict their own uncertainty on the sampled trajectories.
At the same time, the \gls{me}-based safe planners we proposed also suffer from the limitation of many \gls{qd} approaches, namely the need to hand-design the behavior space. 
While some works have been proposed to address this issue \citep{cully2019autonomous, paolo2020unsupervised}, these add another layer of complexity to the system, possibly reducing performance with respect to the safety constraints.


% \gls{name} is a step forward in the direction of applying \gls{rl} approaches to real control engineering systems, providing a powerful yet flexible framework for safe \gls{rl}. 


==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
The results presented in Sec. \ref{sec:results} show how \gls{name} can reach high performances while keeping safety cost low on two of the three environments tested.
As expected, on Acrobot, safe methods reach lower MAR scores compared to unsafe ones due to these last ones ignoring the safety constraints.
At the same time, this leads to much higher $p(\text{unsafe})$ for unsafe approaches.
Interestingly, this is not the case on Pendulum where unsafe approaches tend to have lower MAR scores compared to safe methods even while not respecting safety criteria.
The best unsafe method, ME, has in fact a MAR of $-2.53 \pm 0.19$ while the worst \gls{mbrl} safe method, \gls{mesp}, has a MAR of $-2.27 \pm 0.17$ $(\text{p} < 1e-08)$.
This is likely due to the unsafe region effectively halving the search space.
The left hand side in fact provides lower "safe rewards" compared to the right hand side, pushing the safe algorithms to focus more on swinging the arm towards the right than the left. 
This is particularly visible  %Fig. \ref{fig:exploration}
in Appendices \ref{app:opt} between the safe and unsafe methods where the unsafe area cleanly cuts the distribution of visited states.
Moreover, while the safe methods, and in particular ME cover a larger part of the state space, the safe ones tend to focus much more on the high rewarding state.

When comparing the performances of the different safe planners for \gls{name}, it is possible to notice how the simpler \gls{rss} planner outperforms the more complex \gls{mes} and \gls{mesp} on Pendulum with respect to both MAR $(\text{p}<0.02)$ and $p(\text{unsafe})$ $(\text{p}<0.05)$.
This is not the case on the more complex Acrobot, where the improved search strategies performed by \gls{mes} and \gls{mesp} reach higher MAR scores compared to \gls{rss} $(\text{p} < 0.02)$, while being comparable with respect to the safety cost. This hints at the fact that while a simple strategy like \gls{rss} is very efficient in simple set-ups, more advanced planning techniques are needed in more complex settings. RCEM the closest method to \gls{name}, failed on Pendulum but reached higher MAR on Acrobot, however with twice the safety cost.  

When testing our proposed safe planners on the more challenging SafetyGym environment: Safe Car Goal, we clearly have a gap between simple approaches, \gls{rss} and the more complex ones \gls{mes} and \gls{mesp}.
First, we can see that in terms of MAR no method reach \gls{mes} and \gls{mesp}, not even model-free approaches. 
However, when looking at the  $p(\text{unsafe})$ both methods show to be the most unsafe.  
While both \gls{mes} and \gls{mesp} compare favorably with model-free approaches with respect to the  $p(\text{unsafe})_{trans}$, their $p(\text{unsafe})$ keeps increasing, as shown in Fig. \ref{fig:safecar_results}.
Initially we took 15\% of the total epochs to computed $p(\text{unsafe})_{trans}$ but for the more complex environment the learning of the model take more epochs. This can be explained by the the layout randomization of the Safe Car Goal environment (the hazards positions is randomized at the start of each new episode) which complexity the learning of the model which is required
to generalize in order to safely navigate and solve tasks in different layouts. This effect is supported looking at  \gls{mes} and \gls{mesp} where respectively at around 50k steps  $p(\text{unsafe})$ drops while the reward increases.  


The results also show how model-free approaches require at least one order of magnitude more interactions with the real-system than \gls{mbrl} methods while still having worse MAR scores and higher safety costs.


==> sections/experiments.tex <==
\section{Experimental Setup}
\label{sec:experiments}
We test \gls{name} on two different   OpenAI gym environments with safety constraints (pendulum swing-up, Acrobot )  and the OpenAI safety-gym environment.  In the environment design we follow previous work by \cite{cowen2022samba, ray2019benchmarking} and delegate the details to Appendix C.   




% The environments are shown in Fig. \ref{fig:envs} and described in the following subsections.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=.4\linewidth]{figures/environments.pdf}
%     \caption{Constraint environments used in our experimental setup. (a): Pendulum upright task avoiding unsafe region (red). (b): Acrobot upright task avoiding unsafe region (red).}
%     \label{fig:envs}
% \end{figure}

% These sections can probably be shortened if we need more space




==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
\begin{figure}[ht!]
    \centering
    \includegraphics[width=.6\linewidth]{figures/Acrobot_planning.pdf}
    \caption{An illustrative example of planning with model-based approach on the Acrobot environment. The agent controls the torque on the first joint with the goal of getting its end effector as high as possible, avoiding the unsafe zone (red area). Starting in the rest position (left) the agent uses its model to find the best plan (middle) that will maximize the reward while satisfying the safety constraint and execute it on the real system (right). The example is especially relevant to applications in which safety and reward are traded off.  }
    \label{fig:planning_example}
\end{figure}
In recent years, deep \gls{rl} solved complex sequential decision-making problems in a variety of domains, such as controlling robots, and video and board games \citep{mnih2013playing, andrychowicz2020learning,silver2016mastering}. 
However, in the majority of these cases, success is limited to a simulated world. The application of these RL solutions to real-world systems is still yet to come. 
The main reason for this gap is the fundamental principle of \gls{rl} of learning by trial and error to maximize a reward signal \citep{sutton2018reinforcement}. 
This framework requires unlimited access to the system to explore and perform actions possibly leading to undesired outcomes.  
This is not always possible.
For example, considering the task of finding the optimal control strategy for a data center cooling problem \citep{lazic2018cooling}, the \gls{rl} algorithm could easily take actions leading to high temperatures during the learning process, affecting and potentially breaking the system. 
Another domain where safety is crucial is robotics. 
Here unsafe actions could not only break the robot but could potentially also harm humans. 
This issue, known as \textit{safe exploration}, is a central problem in AI safety \citep{amodei2016concrete}. 
This is why most achievements in \gls{rl} are in simulated environments, where the agents can explore different behaviors without the risk of damaging the real system. 
However, those simulators are not always accurate enough, if available at all, leading to suboptimal control strategies when deployed on the real-system \citep{salvato2021crossing}. 

With the long-term goal of deploying \gls{rl} algorithms on real engineering systems, it is imperative to  overcome those  limitations. 
A straightforward way to address this issue is to develop algorithms that can be deployed directly on the real system that provide guarantees in terms of constraints, such as safety, to ensure the integrity of the system.
This could potentially have a great impact, as many industrial systems require complex decision-making, which efficient \gls{rl} systems can easily provide. 
Going towards this goal, in this paper we introduce \glsfirst{name}, a safe \gls{mbrl} algorithm that learns a model of the system and uses it to plan for a safe course of actions through \gls{mpc} \citep{garcia1989model}.
\gls{name} learns the model in an iterated batch fashion \citep{matsushima2021deployment,kegl2021model}, allowing for minimal real-system interactions. 
This is a desirable property for safe \gls{rl} approaches, as fewer interactions with the real-system mean less chance of entering unsafe states, a condition difficult to attain with model-free safe \gls{rl} methods \citep{achiam2017constrained, ray2019benchmarking, tessler2018reward}. 
Moreover, by learning a model of the system, this allows  flexibility and safety guarantees as using the model we can anticipate unsafe actions before they occur. Consider the illustrative example in Fig.~\ref{fig:planning_example}: the agent, thanks to the model of its dynamics, can perform ``mental simulation'' and select the best plan to attain its goal while avoiding unsafe zones. 
This contrasts with many of the methods in the literature that address the problem of finding a safe course of action through Lagrangian optimization or by penalizing the reward function \citep{webster2021risk, ma2021conservative, cowen2022samba}. 
\gls{name} avoids unsafe situations by discarding trajectories that are deemed unsafe using the model predictions. 
Within this framework, we propose three different safe planners, one based on a simple random shooting strategy and two based on \gls{me} \citep{mouret2015illuminating}, a more advanced \gls{qd} algorithm.
These planners are used to generate, evaluate, and select the safest actions with the highest rewards.
Using divergent-search methods for planning allows the agent to more widely explore the possible courses of actions.
This leads to both a safer and more efficient search, while covering a higher portion of the state space, an important factor when learning a model, given that more exploratory data lead to better models \citep{yarats2022don}.

We test \gls{name} on three different environments.
The presented results highlight how the model and planners can easily find strategies reaching high rewards with minimal costs, even when the two metrics are antithetical, as is the case for the Safe Acrobot environment.
% Moreover, we show how even a simple planner as random shooting can obtain great performances compared to more advanced planning techniques.

To recap, the contributions of the paper are the following: 
% \Jadd{Maybe here we could stress as contribution the use of QD in MBRL method?}
\begin{itemize}
\item We introduce \glsfirst{name}, an \gls{mbrl} method capable of efficiently learning to avoid unsafe states while optimizing the reward;
\item We propose the use of quality-diversity evolutionary methods as \glsfirst{me} as planning techniques in \gls{mbrl} approaches;
\item We present 3 different planners, \gls{rss}, \gls{mes}, \gls{mesp}, that can generate a wide array of action sequences while discarding the ones deemed unsafe during planning.
\end{itemize}

% The rest of the paper is structured as follows.
% In Sec. \ref{sec:related} we present other approaches developed to deal with safety in \gls{rl} algorithms.
% Sec. \ref{sec:background} introduces the background on which \gls{name} is built, while the method itself is presented in Sec. \ref{sec:method}.
% The experimental setting is described in Sec. \ref{sec:experiments} and the results discussed in Sec. \ref{sec:discussion}. % The paper concludes with Sec. \ref{sec:conclusion} in which we describe the impact, the limitations and possible extensions of \gls{name}.

% \Gadd{there is something in the introdction about the way we introduce the necessity of safe rl methods that is not convincing me. I cannot pinpoint it yet tho :)}



==> sections/method.tex <==
\section{Method}
\label{sec:method}
In this work, we use a model of the environment to plan safe trajectories maximizing the reward function.
In many real settings it is possible to assume that the set of unsafe situations is specified by the engineer. 
For this reason we consider that the cost function is given and the cost is calculated from the states the system is in.

In this section, we describe in detail how \gls{name} trains the model and uses the planners.
An overview of the method is presented in Alg. \ref{alg:method}.
The code is available at: \texttt{<URL hidden for review>}.
\begin{algorithm}[!h]
\caption{\glsfirst{name}}\label{alg:method}
\textbf{INPUT:} real-system $p_{\text{real}}$, number of episodes $M$, number of action sequences for planning step $N$, planning horizon length $h$, episode length $T$, initial random policy $\pi^0$\;
\textbf{RESULT:} learned model $p(\cdot)$ and planner\;
Initialize empty trace $\mathcal{T}r = \emptyset$\;
$s_0 \leftlsquigarrow p_{\text{real}}$ \algorithmiccomment{Sample initial state from real system}\\
\For{t in [0, ..., T]}{
$a_t \leftlsquigarrow \pi^0(s_t)$\algorithmiccomment{Generate random action}\\
$\mathcal{T}r = \mathcal{T}r \bigcup (a_t, s_t)$ \algorithmiccomment{Store transition in trace}\\
$s_{t+1} \leftlsquigarrow p_{\text{real}}(s_t, a_t)$\algorithmiccomment{Apply action on real system and get new state}\\
}

\For{i in [1,...,M]}{
$p^i \leftarrow \text{TRAIN}(p^{i-1}, \mathcal{T}r)$ \algorithmiccomment{Train model}\\
\For{t in [0, ..., T]}{
$a_t \leftlsquigarrow \text{PLAN}(p^i, s_t, h, N)$ \algorithmiccomment{Use planner to generate next action}\\
$\mathcal{T}r = \mathcal{T}r \bigcup (a_t, s_t)$\algorithmiccomment{Store transition in trace}\\
$s_{t+1} \leftlsquigarrow p_{\text{real}}(s_t, a_t)$\algorithmiccomment{Apply action on real system and get new state}\\
}
}
\end{algorithm}

\subsection{Training the model}
Let $\mathcal{T}r_t =  \{(s_1,a_1, r_1,c_1,s'_1) ... (s_t,a_t, r_t,c_t,s'_t)\}$ be a system trace consisting of $t$ steps and $(s_t,a_t)$ a state-action tuple. The goal is to train a model $p$ to predict $s_{t+1}$ given the previous $(s_t,a_t)$.
This model can be learned in a supervised fashion given the history trace  $\mathcal{T}r_t$.
We chose as $p$ a deterministic deep mixture density network \citep{bishop1994mixture}, which has proven to have good properties when used in \gls{mpc} \citep{kegl2021model}.
More details on the model parameters and training can be found in Appendix \ref{app:training_details}.


\subsection{Planning for safety}
\label{sec:planners}

The trained model $p(s_t, a_t)$ is used in an \gls{mpc} fashion to select the action $a_{t}$ to apply on the real system.
This means that at every time step $t$ we use the model to evaluate $N$ action sequences by simulating the trajectories of length $h$ from state $s_t$.
For each action sequence, the return $R$ and the cost $C$
\begin{equation}
\label{eq:rew_cost}
    R = \sum_{k=0}^{h} \gamma^k r(\Tilde{s_k}, a_k), \quad C = \sum_{k=0}^{h} \gamma^k c(\Tilde{s_k}, a_k);
\end{equation}
are evaluated, where $\Tilde{s_k}$ is the state generated by the model $p(\cdot)$ and $\gamma$ the discount factor.
\gls{name} then selects the first action of the best sequence, with respect to both the return and the cost.
In this work, we assume that both the reward function $r(s, a)$ and the cost function $c(s, a)$ are given.
In reality, this is not limiting, as in many real engineering settings both the reward and the cost are known and given by the engineer. We tested three different approaches to generate and evaluate safe action sequences at planning time.

\subsubsection{\glsfirst{rss}}

Based on the Random Shooting planner used in \cite{kegl2021model}, \glsfirst{rss} generates $N$ random sequences of actions $a_i \in A$ of length $h$.
These sequences are then evaluated on the model starting from state $s_t$.
The next action $a_t$ to apply on the real system is selected from the action sequence with the lowest cost.
If multiple action sequences have the same cost, $a_t$ is selected from the one with the highest reward among them.
The pseudocode of the planner is shown in Appendix \ref{app:rs}.

\subsubsection{\glsfirst{mes}}
\glsfirst{mes} is a safe version of the \gls{me} algorithm detailed in Appendix \ref{app:me}.
Rather than directly generating sequences of actions as done by \gls{rss}, here we generate the weights $\phi$ of small \glspl{nn} that are then used to generate actions depending on the state provided as input: $\phi(s_t) = a_t$.
This removes the dependency on the horizon length $h$ of the size of the search space present in \gls{rss}.
After the evaluation of a policy $\phi_i$, this is added to the collection $\mathcal{A}_{ME}$.
If another policy with the same behavior descriptor has already been found, \gls{mes} only keeps the policy with the lowest cost.
If the costs are the same, the one with the highest reward will be stored.

Moreover, at each generation, the algorithm samples $K$ policies $\phi$ from the collection to generate $K$ new policies $\Tilde\phi$.
For this step, only the policies with $C = 0$ are considered.
If there are enough policies in the collection satisfying this requirement, the probability of sampling each policy is weighted by its reward.
On the contrary, if only $k < K$ policies with $C = 0$ are in the collection, the missing $K-k$ are randomly generated.
This increases the exploration and can be useful in situations in which it is difficult not to incur in any cost.
The pseudocode of the planner is shown in Appendix \ref{app:mes}.


\subsubsection{\glsfirst{mesp}}
Another safe version of the \gls{me} algorithm.
Contrary to \gls{mes}, which only samples policies for which $C=0$, \gls{mesp} sorts all the policies present in the collection into non-dominated fronts.
The $K$ policies are then sampled from the best non-dominated front.
In case less than $K$ policies are present on this front, \gls{mesp} samples them from the other non-dominated front, in decreasing order of non-domination, until all $K$ policies are selected.

This strategy takes advantage of the search process operated until that point even when not enough safe solutions are present, rather than relying on random policies as done with \gls{mes}.
The pseudo code of the planner is shown in Appendix \ref{app:mesp}.


==> sections/related.tex <==
\section{Related Work}
\label{sec:related}
Some of the most common techniques addressing safety in \gls{rl} rely on solving a \gls{cmdp} \citep{altman1999constrained} through model-free \gls{rl} methods \citep{achiam2017constrained, ray2019benchmarking, tessler2018reward, hsu2021improving, zhang2020first}.
Among these approaches, a well-known method is CPO \citep{achiam2017constrained} which adds constraints to the policy optimization process in a fashion similar to TRPO \citep{schulman2015trust}.
A similar approach is taken by PCPO \citep{yang2020projection} and its extension \citep{yang2020accelerating}.
The algorithm works by first optimizing the policy with respect to the reward and then projecting it back on the constraint set in an iterated two-step process.
A different strategy consists in storing all the ``recovery'' actions that the agent took to leave unsafe regions in a separate replay buffer \citep{hsu2021improving}.
This buffer is used whenever the agent enters an unsafe state by selecting the most similar transition in the safe replay buffer and performing the same action to escape the unsafe state.

Model-free \gls{rl} methods need many interactions with the real-system in order to collect the data necessary for training.
This can be a huge limitation in situations in which safety is critical, where increasing the number of samples increases the probability of entering unsafe states.
\gls{mbrl} limits this problem by learning a model of the system that can then be used to learn a safe policy.
This allows increased flexibility in dealing with unsafe situations, even more if the safety constraints change in time.

Many of these methods work by modifying either the cost or the reward function to push the algorithm away from unsafe areas.
The authors of Uncertainty Guided \gls{cem} \citep{webster2021risk} extend PETS \citep{chua2018deep} by modifying the objective function of the \gls{cem}-based planner to avoid unsafe areas.
In this setting, an unsafe area is defined as the set of states for which the ensemble of models has the highest uncertainty.
A different strategy is to inflate the cost function with an uncertainty-aware penalty function, as done in CAP \citep{ma2021conservative}.
This cost change can be applied to any \gls{mbrl} algorithm and its conservativeness is automatically tuned through the use of a PI controller.
Another approach, SAMBA \citep{cowen2022samba}, uses \gls{gp} to model the environment.
This model is then used to train a policy by including the safety constraint in the optimization process through Lagrangian multipliers.
Closer to \gls{name} are other methods using a trajectory sampling approach to select the safest trajectories generated by \gls{cem} \citep{wen2018constrained, liu2020constrained}. 
This lets us deal with the possible uncertainties of the model predictions that could lead to consider a trajectory safe when it is not.
% \Gadd{From what I understand by reading their paper, this approach is quite similar to ours....}


==> sections/results.tex <==
\section{Experiments}
\label{sec:experiments}
\subsection{Environments}
\label{sec:environments}
We test \gls{name} on two different   OpenAI gym environments with safety constraints (pendulum swing-up, Acrobot) and the OpenAI safety-gym environment \citep{Ray2019}. 
In the environment design we follow previous work \citep{cowen2022samba, ray2019benchmarking} and delegate the details to Appendix \ref{app:envs}.   


\subsection{Results}
\label{sec:results}

We compare \gls{name} with the three different planners introduced in Sec. \ref{sec:planners} against various baselines.
To have a baseline about how much different are the performances of safe methods with respect to unsafe ones, we compared against two unsafe versions of \gls{name}: \textbf{RS} and \textbf{ME}.
\textbf{RS} performs random shooting to plan for the next action, while \textbf{ME} uses vanilla MAP-Elites as a planner, without taking into account any safety requirement.
We also compared against the safe \gls{mbrl} approach \textbf{RCEM} \citep{liu2020constrained} and its respective unsafe version, labeled \textbf{CEM}.
Moreover, to show the efficiency of model-based approaches when dealing with safety requirements, we compared against three model-free baselines: \textbf{CPO} \citep{achiam2017constrained}, \textbf{TRPO lag} and \textbf{PPO lag}; all of them come from the Safety-Gym benchmark \citep{ray2019benchmarking}. 

\begin{figure}[!h]
    \centering
    \subfloat{
       \includegraphics[width=.8\linewidth]{figures/Pendulum_reward.pdf}
       \label{fig:pendulum_reward} 
    }
    \vspace{-0.5cm}

    \subfloat{
       \includegraphics[width=.8\linewidth]{figures/Pendulum_proba_unsafe.pdf}
       \label{fig:pendulun_cost}
    }

    \caption{ Mean reward and probability percentage of unsafe for Safe Pendulum environment. Dashed curves indicate Model-free baselines and plain one Model-based approaches. Thicker lines represent the proposed algorithms. The red dashed line indicates the random unsafe probability.}
    \label{fig:pendulum_results}
\end{figure}

\begin{figure}[!h]
    \centering
    \subfloat{
        \includegraphics[width=.8\linewidth]{figures/Acrobot_reward.pdf}
        \label{fig:acrobot_reward} 
    }
    \vspace{-0.7cm}

    \subfloat{
        \includegraphics[width=0.8\linewidth]{figures/Acrobot_proba_unsafe.pdf}
        \label{fig:acrobot_cost} 
    }
    \caption{Mean reward and probability percentage of unsafe for Safe Acrobot environment. Dashed curves indicate Model-free baselines and plain one Model-based approaches. Thicker lines represent the proposed algorithms. The red dashed line indicates the random unsafe probability.}
    \label{fig:acrobot_results}
\end{figure}
\vspace{-0.5cm}


\begin{figure}[!ht]
    \centering
    \subfloat{
        \includegraphics[width=0.8\linewidth]{figures/SafeCarGoal_reward.pdf}
        \label{fig:safecar_reward} 
    }
    \vspace{-0.5cm}

    \subfloat{
        \includegraphics[width=0.8\linewidth]{figures/SafeCarGoal_cost.pdf}
        \label{fig:safecar_cost} 
    }
    \caption{Mean reward and probability percentage of unsafe for Safe Car Goal environment. Dashed curves indicate Model-free baselines and plain one Model-based approaches. Thicker lines represent the proposed algorithms. The red dashed line indicates the random unsafe probability.}
    \label{fig:safecar_results}
\end{figure}

\begin{table}[!ht]
\caption{Summary of the different methods on the two different environments Pendulum and Acrobot. MAR is the mean asymptotic reward, MRCP($r_{thr}$) is the number of system  access steps needed to achieve $r_{thr}$ of the optimum reward, $p(\text{unsafe})[\%]$ and  $p(\text{unsafe})[\%]_{trans}$ are the probability percentage of being unsafe during epochs. All the metrics are average over all epochs and seeds and $\downarrow$ and $\uparrow$ mean lower and higher the better, respectively. The best \textbf{safe methods} with respect to each metric are highlighted in bold. All $\pm$ values are 90\% Gaussian confidence interval.}
\centering
\begin{tabular}{
l
l@{$ \hspace{0.1cm} \pm \hspace{0.1cm}$}l
l@{$ \hspace{0.1cm} \pm \hspace{0.1cm} $}l
l@{$ \hspace{0.1cm} \pm \hspace{0.1cm} $}l
c@{$ \hspace{0.05cm} \pm \hspace{0.1cm} $}l
}
\toprule
Method & \multicolumn{2}{c}{MAR $\uparrow$} & \multicolumn{2}{c}{MRCP$\times10^3 \downarrow$} & \multicolumn{2}{c}{$p(\text{unsafe})[\%] \downarrow$} &  \multicolumn{2}{c}{$p(\text{unsafe})_{trans} [\%] \downarrow$} \\ \midrule
                      & \multicolumn{8}{c}{Safe Pendulum $r_{thr} = -2.5$ }                                                                 \\ \cmidrule(l){2-9} 
\gls{name}(\gls{rss})   &   \textbf{-2.09}&\textbf{0.09}    &   2.12&1.45   &   \textbf{0.35}&\textbf{0.63} &   1.23&1.28   \\
\gls{name}(\gls{mes})   &   -2.2&0.16   &   \textbf{2.0}&\textbf{0.9}   &   0.63&0.57   &   \textbf{0.54}&\textbf{0.57} \\
\gls{name}(\gls{mesp})  &   -2.27&0.17  &   2.10&1  &   0.58&0.52   &   0.6&0.56 \\
RCEM            & -6.12 &  0.15          & 6.7 & 0.81          & 0.63 &  0.64                  & 0.84 &  0.7                             \\
\cmidrule(l){2-9}
RS &    -2.7&0.14   &   2.60&1.2    &   1.49&1.0    &   1.36&0.61 \\
\gls{me}    &   -2.53&0.19  &   1.90&0.7    &   3.01&2.78   &   2.01&1.95 \\
CEM &   -2.99&0.15 &   1.64&0.41  &   1.59&0.89   &   1.43&0.85 \\
\cmidrule(l){2-9}
CPO             & -6.06 &  0.04         & 22 &  0.0         & 1.73 &  0.92                  & 1.59 &  0.78                             \\
PPO  lag        & -4.1 &  0.12          & 138 &  65       & 2.05 &  1.75                  & 2.15 &  1.48                             \\
TRPO lag        & -7.02 &  0.03         & 161 &  55       & 1.31 &  0.91                  & 2.07 &  0.89  \\
& \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}            & \multicolumn{1}{l}{} \\

                        & \multicolumn{8}{c}{Safe Acrobot $r_{thr} = 1.6$}                                                 \\
                        \cmidrule(l){2-9} 
\gls{name}(\gls{rss})        & 1.35 & 0.07     & 1.6  & 0.26      & \textbf{1.1}         & \textbf{1.05}       & \textbf{1.85}                   & \textbf{1.56}                  \\
\gls{name}(\gls{mes})   &   1.64&0.01   &   \textbf{1.36}&\textbf{0.25} &   \textbf{1.1}&\textbf{1.22}  &   2.45&1.92 \\
\gls{name}(\gls{mesp})  &   1.65&0.01 &   1.56&0.11   &   1.42&1.62   &   3.75&2.77 \\
RCEM                          &\textbf{ 1.68} & \textbf{0.01}     &  1.60  & 0.37        & 2.01         & 1.4        & 2.85                    & 1.84                   \\
\cmidrule(l){2-9} 
RS              & 2.07 & 0.01     & 1.28 & 0.29     & 24.8        & 8.3        & 10.85                  & 7.36                  \\
\gls{me}    &   2.12&0.02   &   1.12&0.24  &   25.6&7.91   &   12.18&7.95 \\
CEM                           & 2.12 & 0.02     &  1.40    &   0.43        & 24.9        & 8.91       & 9.14                   & 7.17                  \\
\cmidrule(l){2-9} 
CPO                           & 0.94 & 0.01     & 87 & 59    & 5.43        & 1.74       & 4.35                   & 2.49                  \\
PPO  lag               & 0.94 & 0.01     & 24 & 3     & 3.7         & 1.94       & 4.02                   & 2.46                  \\
TRPO  lag              & 1.02 & 0.01     & 37 & 22    & 4.2        & 2.0        & 4.31                   & 2.53     \\  
& \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}            & \multicolumn{1}{l}{} \\

                        & \multicolumn{8}{c}{Safe Car Goal $r_{thr} = 10$}                                                 \\
                        \cmidrule(l){2-9} 
\gls{name}(\gls{rss})        & -0.29 & 0.22     & -  & -      & 0.72        & 1.05      & 0.44                   & 0.81                  \\
\gls{name}(\gls{mes})   &   \textbf{14.65} & \textbf{1.90} &   32 & 0.0  &  2.10 & 3.64   & \textbf{0.35} & \textbf{0.56} \\
\gls{name}(\gls{mesp})  &   9.80 & 1.73 &   \textbf{12.33} & \textbf{4.54}  &   1.99 & 2.80  & 0.50 & 0.78 \\
RCEM                    &   -1.41 & 0.21 & - & -   & \textbf{ 0.50} & \textbf{0.83}   &  0.63 & 0.99 \\
\cmidrule(l){2-9} 
% RS              & 2.07 & 0.01     & 1.28 & 0.29     & 24.8        & 8.3        & 10.85                  & 7.36                  \\
% \gls{me}    &   -&-   &   -&-  &   -&-   &  -&- \\
CEM                    & 0.94 & 2.06 &  50 & 0.0  & 1.17 & 2.47       & 0.67 & 1.26 \\ 
\cmidrule(l){2-9} 

CPO                 & 3.95 & 0.09     &  297 & 153.6     & 0.55  & 1.11       & 0.42 & 0.68  \\
PPO  lag            & 5.36 & 0.1     &  231 &  121.24    & 0.66  & 1.51       & 0.34 & 0.58  \\
TRPO  lag           & 3.66 & 0.07     & 108    & 0.0     & 0.65  & 1.58        & 0.39 & 0.72     \\ \bottomrule 

\end{tabular}

\label{tab:metrics_table}
\end{table}

The algorithms are compared according to four metrics: Mean Asymptotic Reward (\textbf{MAR}), Mean Reward Convergence Pace (\textbf{MRCP}),  Probability percentage of unsafe (\textbf{p(unsafe)[\%]}) and transient probability percentage of unsafe (\textbf{p(unsafe)[\%]$_{trans}$}).
The details on how these metrics are calculated are defined in Appendix \ref{app:metrics}.

% \begin{table}[!h]
% \caption{Summary of the different methods on the two different environments Pendulum and Acrobot. MAR is the mean asymptotic reward, MRCP($r_{thr}$) is the number of system  access steps needed to achieve $r_{thr}$ of the optimum reward, $p(\text{unsafe})[\%]$ and  $p(\text{unsafe})[\%]_{trans}$ are the probability percentage of being unsafe during epochs. All the metrics are average over all epochs and seeds and $\downarrow$ and $\uparrow$ mean lower and higher the better, respectively. The best \textbf{safe methods} with respect to each metric are highlighted in bold.}
% \centering
% \begin{tabular}{
% l
% l@{$ \hspace{0.1cm} \pm \hspace{0.1cm}$}l
% l@{$ \hspace{0.1cm} \pm \hspace{0.1cm} $}l
% l@{$ \hspace{0.1cm} \pm \hspace{0.1cm} $}l
% c@{$ \hspace{0.05cm} \pm \hspace{0.1cm} $}l
% }
% \toprule
% Method & \multicolumn{2}{c}{MAR $\uparrow$} & \multicolumn{2}{c}{MRCP$\times10^3 \downarrow$} & \multicolumn{2}{c}{$p(\text{unsafe})[\%] \downarrow$} &  \multicolumn{2}{c}{$p(\text{unsafe})_{trans} [\%] \downarrow$} \\ \midrule
%                       & \multicolumn{8}{c}{Pendulum $r_{thr} = -2.5$ }                                                                 \\ \cmidrule(l){2-9} 
% \gls{name}(\gls{rss})   &   \textbf{-2.09}&\textbf{0.09}    &   2.12&1.45   &   \textbf{0.35}&\textbf{0.63} &   1.23&1.28   \\
% \gls{name}(\gls{mes})   &   -2.2&0.16   &   \textbf{2.0}&\textbf{0.9}   &   0.63&0.57   &   \textbf{0.54}&\textbf{0.57} \\
% \gls{name}(\gls{mesp})  &   -2.27&0.17  &   2.10&1  &   0.58&0.52   &   0.6&0.56 \\
% RS &    -2.7&0.14   &   2.60&1.2    &   1.49&1.0    &   1.36&0.61 \\
% \gls{me}    &   -2.53&0.19  &   1.90&0.7    &   3.01&2.78   &   2.01&1.95 \\
% CEM &   -2.99&0.15 &   1.64&0.41  &   1.59&0.89   &   1.43&0.85 \\
% RCEM            & -6.17 &  0.1          & inf & inf          & 0.73 &  0.75                  & 0.64 &  0.54                             \\
% CPO             & -6.06 &  0.04         & 22 &  0.0         & 1.73 &  0.92                  & 1.59 &  0.78                             \\
% PPO  lag        & -4.1 &  0.12          & 138 &  65       & 2.05 &  1.75                  & 2.15 &  1.48                             \\
% TRPO lag        & -7.02 &  0.03         & 161 &  55       & 1.31 &  0.91                  & 2.07 &  0.89  \\
% & \multicolumn{1}{l}{}    & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{}            & \multicolumn{1}{l}{} \\

%                         & \multicolumn{8}{c}{Acrobot $r_{thr} = 1.6$}                                                 \\
%                         \cmidrule(l){2-9} 
% \gls{name}(\gls{rss})        & 1.35 & 0.07     & 1.6  & 0.26      & \textbf{1.1}         & \textbf{1.05}       & \textbf{1.85}                   & \textbf{1.56}                  \\
% \gls{name}(\gls{mes})   &   1.64&0.01   &   \textbf{1.36}&\textbf{0.25} &   \textbf{1.1}&\textbf{1.22}  &   2.45&1.92 \\
% \gls{name}(\gls{mesp})  &   \textbf{1.65}&\textbf{0.01} &   1.56&0.11   &   1.42&1.62   &   3.75&2.77 \\
% RS              & 2.07 & 0.01     & 1.28 & 0.29     & 24.8        & 8.3        & 10.85                  & 7.36                  \\
% \gls{me}    &   2.12&0.02   &   1.12&0.24  &   25.6&7.91   &   12.18&7.95 \\
% CEM                           & 2.12 & 0.02     &  1.40    &   0.43        & 24.9        & 8.91       & 9.14                   & 7.17                  \\
% RCEM                          & 0.13 & 0.01     &  inf  & inf        & 0.0         & 0.0        & 0.0                    & 0.0                   \\
% CPO                           & 0.94 & 0.01     & 87 & 59    & 5.43        & 1.74       & 4.35                   & 2.49                  \\
% PPO  lag               & 0.94 & 0.01     & 24 & 3     & 3.7         & 1.94       & 4.02                   & 2.46                  \\
% TRPO  lag              & 1.02 & 0.01     & 37 & 22    & 4.2        & 2.0        & 4.31                   & 2.53     \\ \bottomrule 
% \end{tabular}

% \label{tab:metrics_table}
% \end{table}

% \vspace{-4cm}

The results are shown in Table \ref{tab:metrics_table}.
The MAR scores and the $p(\text{unsafe})[\%]$ for the pendulum system are shown in Fig. \ref{fig:pendulum_results}, while the ones for the acrobot system are in Fig. \ref{fig:acrobot_results}. Finally, Fig. \ref{fig:safecar_results} shows the results for the Safe\_Car\_Goal environment.
% the  shows the visited states distributions for the Safe Pendulum environment.
Additional plots are presented in Appendices \ref{app:opt} and \ref{app:exp}.

